Measuring third party tracker power across web and mobile

Third-party networks collect vast amounts of data about users via web sites and mobile applications. Consolidations among tracker companies can significantly increase their individual tracking capabilities, prompting scrutiny by competition regulators. Traditional measures of market share, based on revenue or sales, fail to represent the tracking capability of a tracker, especially if it spans both web and mobile. This paper proposes a new approach to measure the concentration of tracking capability, based on the reach of a tracker on popular websites and apps. Our results reveal that tracker prominence and parent-subsidiary relationships have significant impact on accurately measuring concentration.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> bigtables.tex <==
\begin{table}[tbp] %!h
\centering
\small
\begin{tabular}{c|c|P{1.7in}|P{1.9in}}\\
\textbf{Tracker} & \textbf{Jurisdiction} & \textbf{Number/Ranking of presence in web sites} & \textbf{Number and Ranking of presence in mobile apps} \\\hline
Google & us & 3676 (1) & 4444 (1) \\
Facebook & us & 1898 (2) & 1274 (3) \\
Amazon & us & 1187 (3) & 55 (36) \\
\textbf{comscore} & us & 999 (4) & 105 (4) \\
Twitter & us & 865 (6) & 82 (25) \\
Adobe & us & 767 (8) & 138 (22) \\
\textbf{Yahoo} & us & 662 (10) & 229 (21) \\
\textbf{AOL} & us & 642 (11) & 303 (35) \\
Rubicon & us & 474 (17) & 189 (16) \\
\textbf{Opsmatic(NewRelic)} & us & 419 (22) & 47 (42) \\
Yandex & ru & 201 (49) & 64 (31) \\
\textbf{microsoft} & us & 198 (51) & 142 (44) \\
Baidu & cn & 147 (57) & 26 (65) \\
Smartadserver & fr & 142 (60) & 33 (59) \\
Mixpanel & us & 81 (91) & 72 (30) \\
\textbf{Alibaba(umeng)} & cn & 109 (83) & 126 (23) \\
mail.ru & ru & 56 (119) & 75 (27) \\
\textbf{Spearhead (Smaato)} & us & 42 (165) & 46 (44) \\
Tencent & cn & 26 (236) & 61 (33) \\
Weibo & cn & 18 (326) & 37 (53) \\
Applovin & us & 17 (349) & 420 (11) \\
Ironsource & us & 2 (1606) & 144 (19) \\
Inmobi & us & 3 (1319) & 528 (8)\\ 
Appboy & us & 3 (1422) & 35 (57) \\
Mobfox & us & 2 (2018) & 32 (60) \\\hline
\end{tabular}
\end{table}\label{table:overlap}

\begin{table}[h!] %!h
\parbox{.45\linewidth}{
\centering
\small
\begin{tabular}{c|c|P{1in}}\\
\textbf{Tracker} & \textbf{Juris.} & \textbf{Prevalence}  \\\hline
Google 			& us & 256 \\
Doubleclick 		& us & 233 \\
Facebook 			& us & 168 \\
Scorecardresearch	& us & 91 \\
Appnexus			& us & 85 \\
Criteo			& fr & 68 \\
Adobe			& us & 61 \\
Yahoo			& us & 59 \\
Twitter			& us & 59 \\
Cloudfront			& us & 57 \\
\end{tabular}
}
\hfill
\parbox{.45\linewidth}{
\centering
\small
\begin{tabular}{c|c|P{1in}}\\
\textbf{Tracker} & \textbf{Juris.} & \textbf{Prevalence}  \\\hline
google		& us & 286 \\
facebook		& us & 172 \\
crashlytics		& us & 151 \\
fabric		& us & 137 \\
comscore		& us & 48 \\
twitter		& us & 42 \\
bitstadium		& us & 34 \\
urbanairship	& us & 24 \\
mopub		& us & 22 \\
card.io		& us & 17 \\
\end{tabular}
}
\end{table}\label{table:overlap}





==> exiting-analysis.tex <==
\subsection{alternative measures trackers by integration and company tracing}

Purpose and findings of existing analysis

== Web tracker analysis ==

Web tracking has been extensively studied over the years. Past research has consistently demonstrated the continuous growth and prevalence of third party tracking on web sites.  Furthermore, domination of tracking behaviours by several leading companies have been also repeatedly observed and confirmed [Roesner 2012, Libert 2015, Yu 2016, Ren 2016]. For example, Roesner et al observed that ``several trackers can each capture more than 20\% of a user?s browsing behavior'', and the study by Ren et al. over 1 million web sites also showed that only a fraction of the 81,000 web trackers they identified are present in over 10k web sites.  A more recent field study by Yu et al provided a finer-grained view into tracker behaviour, by analysing the safe v.s. unsafe data being transmitted to and from trackers. They results showed that the prevalence of tracking is slightly lower if we consider whether unsafe data are actually accessed by the trackers. However, tracking is still a prevalent and wide spread phenomena, spanning across all types of web sites. 

Various approaches have also been applied to quantify the prominence and impact of trackers. Princton defines a prominence metric for measuring the prominence of third party trackers, which takes into consideration the ranking of the web sites in which the trackers appeared.  In this way, they were able to calculate the prominence of a tracker without replying on a large scale we tracking data. /// other quantification metric // However, none of these studies have tried to quantify the degree of impact on users' privacy detriment by the distribution of trackers in the web tracking ecosystem. 

To be reviewed further: web tracking census // tracking the trackers [yu www2016]: // tracking the trackers (haystack)

%Roesner 2012: one of the early stage work on identify the different types of tracking behaviours on the web, by studying xxx web sites. the study also identity the tracking concentration behaviour back in 2012, where the authors observed that 
%Princeton: measure web tracking at a large scale. The presence of trackers is long tail and their prevalence quickly drops off. Trackers on the tail are present in very few web sites that are very likely to be encountered by average users. Those on the head of the tail are however concentrated around a few large dominating companies, who bring a much larger privacy impact on average users. 

== Mobile tracker analysis == 

== Combine analysis == 

= Methodology = 

There are two major ways to collect web tracking information: crowd-sourcing (\$heriff, Bobble) or simulated user interactions (Princeton, FPDetecive). 

We use OpenWPM because it supports both stateful and stateless web tracking measurements, requires no native browser code to be deployed, and it also makes its web tracking data open accessible.

= Scale =
